The Index of Invariance and its Implications for a Parameterized Least Squares Problem

We study the problem $x_{b,\omega} := \text{arg min}_{x \in \mathcal{S}} \|(A + \omega I)^{-1/2} (b - Ax)\|_2$, with $A = A^*$, for a subspace $\mathcal{S}$ of $\mathbb{F}^n$ ($\mathbb{F} = \mathbb{R}$ or $\mathbb{C}$), and $\omega > -\lambda_{min}(A)$. We show that there exists a subspace $\mathcal{Y}$ of $\mathbb{F}^n$, independent of $b$, such that $\{x_{b,\omega} - x_{b,\mu} \mid \omega,\mu > -\lambda_{min}(A)\} \subseteq \mathcal{Y}$, where $\dim(\mathcal{Y}) \leq \dim(\mathcal{S} + A\mathcal{S}) - \dim(\mathcal{S}) = \mathbf{Ind}_A(\mathcal{S})$, a quantity which we call the index of invariance of $\mathcal{S}$ with respect to $A$. In particular if $\mathcal{S}$ is a Krylov subspace, this implies the low dimensionality result of Hallman & Gu (2018). The problem is also such that when $A$ is positive and $\mathcal{S}$ is a Krylov subspace, it reduces to CG for $\omega = 0$ and to MINRES for $\omega \to \infty$. We study several properties of $\mathbf{Ind}_A(\mathcal{S})$ in relation to $A$ and $\mathcal{S}$. We show that the dimension of the affine subspace $\mathcal{X}_b$ containing the solutions $x_{b,\omega}$ can be smaller than $\mathbf{Ind}_A(\mathcal{S})$ for all $b$. However, we also exhibit some sufficient conditions on $A$ and $\mathcal{S}$, under which $\mathcal{X} := \text{Span}{\{x_{b,\omega} - x_{b,\mu} \mid b \in \mathbb{F}^n, \omega,\mu > -\lambda_{min}(A)\}}$ has dimension equal to $\mathbf{Ind}_A(\mathcal{S})$. We then study the injectivity of the map $\omega \mapsto x_{b,\omega}$, leading us to a proof of the convexity result from Hallman & Gu (2018). We finish by showing that sets such as $M(\mathcal{S},\mathcal{S}') = \{A \in \mathbb{F}^{n \times n} \mid \mathcal{S} + A\mathcal{S} = \mathcal{S}'\}$, for nested subspaces $\mathcal{S} \subseteq \mathcal{S}' \subseteq \mathbb{F}^n$, form smooth real manifolds, and explore some topological relationships between them.

==> archive/defn-notation-old.tex <==
\subsection{Definitions and notation}
\label{ssec:defn}

All relevant definitions and notations to be used throughout the paper are introduced here. Some additional concepts of topology and real analytic functions are required in \Cref{sec:converse,sec:related-results}, which we don't introduce below for brevity; but we use standard terminology. The unfamiliar reader is referred to textbooks on these topics such as \cite{rudin1964principles, armstrong2013basic}. In \Cref{sec:related-results} we have a couple of results on smooth manifold embeddings, and we use terminology consistent with \cite{lee2013smooth}. We use $\F$ to represent the field we work over, which can be either $\C$ or $\R$.

\subsubsection{Matrix notations}
\label{sssec:hilbert-spaces}

Let $\H$ be a finite dimensional Hilbert space over $\F$, and let $\dim{\H} = n \geq 1$. If $\F = \C$, we assume that the inner product on $\H$ is conjugate linear in the first slot. By choosing an orthonormal basis set $\mathcal{B}$ for $\H$, one can identify $\H$ isometrically with the Hilbert space $\Fn$ equipped with the standard Euclidean inner product, i.e. for $x, y \in \Fn$ the inner product of $x$ and $y$ is defined as $\langle x, y \rangle := \sum_{i=1}^{n} x_i y_i$ when $\F = \R$, and $\langle x, y \rangle := \sum_{i=1}^{n} \overline{x_i} y_i$ when $\F = \C$ (here $\overline{x_i}$ denotes the complex conjugate of $x_i$, and $x_i$ (resp. $y_i$) is the $i^{th}$ element of $x$ (resp. $y$)). We will also use the abbreviated notation $x^\ast y$ to denote $\langle x,y \rangle$. The $\ell^2$-norm of an element $x \in \Fn$ is defined as $\|x\|_2 := \sqrt{x^* x}$. With the chosen orthonormal basis $\mathcal{B}$, each element of $\text{Hom}(\H, \H)$ is uniquely represented by an element of $\Fnn$, which is the vector space of all $n \times n$ matrices over the field $\F$. In fact the identification of $\text{Hom}(\H, \H)$ and $\Fnn$ is also an isometry under the Hilbert-Schmidt inner product. In this paper we only work in the finite dimensional setting --- thus in the rest of the paper it will suffice to assume that $\H = \Fn$, and $\text{Hom}(\H,\H) = \Fnn$, because of the identifications mentioned above.

In many places in this paper we will be working with non-square matrices. Thus we define $\Fpq{p}{q}$ to be the set of all $p \times q$ matrices with $\F$-valued entries. Given any $A \in \Fpq{p}{q}$, we will use the notation $\Img{A}$ to denote its \textit{range}, i.e. $\Img{A} := \{Ax \mid x \in \Fp{q}\}$. The \textit{rank} of $A$ is defined as the dimension of its range, and we denote this as $\rank(A)$. $A$ is said to be \textit{full rank} if $\rank(A)=\min (p,q)$. The adjoint of $A$ is denoted by $A^\ast$, and it is the complex conjugate transpose (resp. transpose) of $A$ when $\F = \C$ (resp. $\R$). $\overline{A}$ will denote the complex conjugate of $A$ without the transpose. A matrix $A \in \Fpq{p}{q}$ is said to be \textit{semi-unitary} if all its columns are orthonormal, i.e. $A^\ast A = I$ (this requires $p \geq q$). Often we will refer to matrices as simply \textit{operators}. 

If $A \in \Fnn$,  $A$ is said to be \textit{Hermitian} if $A = A^\ast$. When $\F = \C$, $A$ is said to be \textit{positive} if $x^\ast Ax > 0$ (i.e. real and positive) for all non-zero $x \in \Fn$ (this in fact ensures that $A$ is Hermitian), while if $\F = \R$ we additionally require that $\F$ is Hermitian. We say that $A$ is \textit{unitary} if $A^\ast A = I$, where $I \in \Fnn$ denotes the identity matrix, which also implies $AA^\ast = I$. The symbol $I$ will be used to denote square identity matrices of other shapes as well, but the shape will always be clear from context. The set of all Hermitian matrices, positive matrices, unitary matrices, and invertible matrices in $\Fnn$ will be denoted using the symbols $\Sym{n}$, $\Pos{n}$, \Uni{n}, and $\Gl{n}$ respectively, and recall that $\Pos{n}\subseteq \Gl{n}$ and $\Uni{n} \subseteq \Gl{n}$ (whether $\F = \R$ or $\C$ will either be clear from context, or will be explicitly stated when there is any chance of confusion). We recall that Hermitian matrices have real eigenvalues and positive matrices have positive eigenvalues. For any $A \in \Sym{n}$, $\evalmin{A}$ will denote its smallest eigenvalue. We also recall that if $A \in \Sym{n}$, then it admits a spectral decomposition $A = U \Lambda U^\ast$ for some $U \in \Uni{n}$ and a real diagonal matrix $\Lambda \in \Fnn$, which allows us to define\footnote{The spectral decomposition guarantees that $\Lambda$ has positive diagonal entries, and is unique up to conjugation by permutation matrices --- so $A^q$ defined this way is unique.} whenever $A \in \Pos{n}$, its power $A^q := U \Lambda^q U^\ast \in \Pos{n}$ for any $q \in \R$, where $(\Lambda^q)_{ij} = \Lambda_{ij}^q$ (sign always chosen to be positive) for all $1 \leq i,j \leq n$.

We also introduce block matrix and vec notation. Firstly \green{LC: should be square ?} for any $A \in \Fnn$, and for any $1 \leq k \leq l \leq n$ and $1 \leq k' \leq l' \leq n$, we will define the block matrix $A_{k:l,k':l'} \in \Fpq{(l-k+1)}{(l'-k'+1)}$ as
\begin{equation}
    \left( A_{k:l,k':l'} \right)_{ij} = A_{k+i-1, k'+j-1}, \;\; \forall \;\; 1 \leq i \leq (l-k+1),  1 \leq j \leq (l'-k'+1).
\end{equation}
Secondly, we define the function $\text{vec}: \F^{m \times n} \to \F^{mn}$ by $\vec{A}_{i+(j-1)m} = A_{ij}$, where $1 \leq i \leq m$, and $1 \leq j \leq n$. Informally, $\vec{A}$ stacks the columns of $A$ on top of each other into a vector. 

\green{For completeness, we define the span of 0 vectors to be $\{0\}$.}
\green{Similarly, if $A \in \F^{m \times p}, B \in \F^{p \times n}$ and $C = AB$, if $p = 0$ we define $C = 0 \in \F^{m \times n}$.}


\subsubsection{Subspaces and affine subspaces}
\label{sssec:affine-subspaces}

A \textit{subspace} $\S$ of $\Fn$ is a subset that is also a $\F$-vector space. An \textit{affine subspace} $\T$ of $\Fn$ is a set satisfying the property that for any $x \in \T$, the set $\S_x := \{x - y \mid y \in \T\}$ is a subspace of $\Fn$. It is easily seen that if $x, x' \in \T$ are distinct then $\S_x = \S_{x'}$, so one can unambiguously associate a subspace $\S := \{x - y \mid y \in \T\}$ with the affine subspace $\T$, where $x \in \T$ is any arbitrarily chosen point. The dimension of $\T$ is defined as the dimension of $\S$ under this association, i.e. $\dim{\T}:= \dim{\S}$. We will use the notation $\Gra{k}{n}$ (resp. $\Gr{k}{n}$)\footnote{$\Gra{k}{n}$ is known as the \textit{complex affine Grassmanian} (resp. \textit{affine Grassmanian}), and $\Gr{k}{n}$ is known as the \textit{complex Grassmanian} (resp. \textit{Grassmanian}), when $\F=\C$ (resp. $\F = \R$).} to denote the set of all $k$-dimensional affine subspaces (resp. subspaces) of $\Fn$. If one defines $x_0 := \argmin_{x \in \T} \norm{x}{2}$ (this minimizer exists\footnote{Existence follows by choosing any point $x \in \T$ and defining the compact set $\T_1 := \{y \in \T \mid \norm{y}{2} \leq \norm{x}{2}\}$, which has the property that for any $y \in \T \setminus \T_1$, $\norm{y}{2} > \norm{x}{2}$, and so the minimization can be performed over $\T_1$.} and is unique because in the case $\F=\C$, if $\Cn \ni x = x_1 + i x_2$ with $x_1, x_2 \in \Rn$, the map $(x_1,x_2) \mapsto \norm{x}{2}^2$ is smooth and strictly convex, while if $\F = \R$, the map $\Rn \ni x \mapsto \norm{x}{2}^2$ is also smooth and strictly convex), it follows that every $\T \in \Gra{k}{n}$ can be represented uniquely as
\begin{equation}
\label{eq:graff-to-gr}
\T = x_0 + \S := \{x_0 + y \mid y \in \S\},
\end{equation}
where
$\S \in \Gr{k}{n}$, $x_0 \in \T$, and $\norm{x_0}{2} \leq \norm{x}{2}$ for all $x \in \T$, which we will call the \textit{normal representation} of $\T$. It will be useful for us to represent the subspace $\S$ appearing in \eqref{eq:graff-to-gr} by the map $\mathbf{\Gamma}_k: \Gra{k}{n} \rightarrow \Gr{k}{n}$, which is the \textit{bundle projection map} viewing $\Gra{k}{n}$ as a \textit{vector bundle} over $\Gr{k}{n}$ \cite{lim2020affinegrass}; thus we can rewrite \eqref{eq:graff-to-gr} as $\T = x_0 + \Gam{k}{\T}$. We note that an affine subspace $\T$ is a subspace if and only if $x_0 = 0$ in its representation \eqref{eq:graff-to-gr}. We also define $\G{n} := \bigcup_{k=0}^{n} \Gr{k}{n}$ (resp. $\Ga{n} := \bigcup_{k=0}^{n} \Gra{k}{n}$) which is the set of all subspaces (resp. affine subspaces) of $\Fn$. Notice that we have the set inclusions $\G{n} \subseteq \Ga{n}$, and $\Gr{k}{n} \subseteq \Gra{k}{n}$ for all $0 \leq k \leq n$. Thus the restriction of the map $\mathbf{\Gamma}_k$ to $\Gr{k}{n}$ is the identity map.

If $\S$ is a subspace of $\Fn$, and $A \in \Fnn$, we define the set $A\S := \{Ax \mid x \in \S\}$, which is simply the image of $\S$ under $A$. Similarly if $\T$ is an affine subspace of $\Fn$, we analogously define $A\T := \{Ax \mid x \in \T\}$. It can be checked that $A\S$ (resp. $A\T$) is a subspace (resp. affine subspace) of $\Fn$. If $\S, \S'$ are subspaces of $\Fn$, we define their sum as $\S + \S' := \{x + y \mid x \in \S, y \in \S'\}$. In a few places in this paper, we will need to consider uncountable sums of subspaces. If $\mathcal{U} \in 2^{\G{n}}$ is a union of subspaces of $\Fn$ (possibly uncountable), we define $\sum \mathcal{U} = \bigl \{ \sum_{i=1}^{m} x_i \mid x_i \in \S \in \mathcal{U}, \; m \geq 0 \text{ and finite} \bigr \}$, and it follows that it is a subspace. When $\S \cap \S' = \{0\}$, the sum is a \textit{direct sum}, which will be denoted as $\S \oplus \S'$. We recall that direct sums have the important property: any $x \in \S \oplus \S'$ can be written uniquely as $x = y + z$, for $y \in \S$ and $z \in \S'$; and conversely if $y_1, y_2 \in \S$ and $z_1, z_2 \in \S'$, with either $y_1 \neq y_2$ or $z_1 \neq z_2$, then $y_1 + z_1 \neq y_2 + z_2$. Intersections of subspaces (resp. affine subspaces), possibly uncountable, is a subspace (resp. affine subspace) of $\Fn$. For any subset $\mathcal{X} \subseteq \Fn$, the \textit{affine hull} $\Aff{\mathcal{X}}$ of $\mathcal{X}$ is the intersection of all affine subspaces (or equivalently the smallest affine subspace) of $\Fn$ containing $\mathcal{X}$, and hence is also an affine subspace. We will define the \textit{affine dimension} of $\mathcal{X}$ to be the dimension of its affine hull. Similarly, the \textit{linear hull} of $\mathcal{X}$, which we denote $\Span{\mathcal{X}}$, is the intersection all subspaces (or equivalently the smallest subspace) of $\Fn$ containing $\mathcal{X}$.
When $A \in \Fpq{p}{q}$, the linear hull of the set of its columns equals its range $\Img{A}$. For $A \in \Fnn$, $b \in \Fn$, and $\mathbb{Z} \ni k \geq 1$, we define the \textit{complex Krylov subspace} (resp. \textit{real Krylov subspace}) $\K_k(A,b) := \Span{\{b, Ab, \dots, A^{k-1}b\}}$ for $\F = \C$ (resp. $\F = \R$). If $\S$ is a subspace, we define its \textit{orthogonal complement} as $\S^{\perp} := \{x \in \Fn \mid x^\ast y = 0, \; \forall \; y \in \S \}$, which is also a subspace.

\subsubsection{Index of invariance}
\label{sssec:index}

We now introduce the most important quantity relevant for this paper which plays a key role in the proofs.

\begin{definition}
\label{def:index}
Let $A \in \Fnn$, and $\S \in \G{n}$ be a subspace of $\Fn$. We define the \textit{index of invariance} of $\S$ with respect to $A$ to be the codimension of $\S$ in $\S + A\S$. Formally we will represent this quantity as a map $\textbf{Ind} : \G{n} \times \Fnn \rightarrow \mathbb{Z}_{\geq 0}$, and so $\Ind{\S}{A} := \dim{\S + A\S} - \dim{S}$. In most of our applications $A$ will be fixed, in which case we will use the compressed notation $\Indsimple{A}{\S}$ to mean $\Ind{\S}{A}$, and treat it as a map $\textbf{Ind}_{A}: \G{n} \rightarrow \mathbb{Z}_{\geq 0}$. In this setting, we will refer to $\Indsimple{A}{\S}$ as simply the \textit{index} of $\S$.
\end{definition}

If $A \in \Fnn$, a subspace $\S \in \G{n}$ is called an \textit{invariant subspace} of $A$ or simply $A-$\textit{invariant} if $A\S \subseteq \S$. Thus it can be seen from \Cref{def:index} that $\Ind{\S}{A} = 0$ if and only if $\S$ is $A-$invariant. Another interesting example is that of a Krylov subspace $\K_k(A,b)$ that is not $A-$invariant, in which case it can be verified that $\Ind{\K_k(A,b)}{A} = 1$. We study several interesting properties of the index of invariance below in \Cref{ssec:properties-index}.

\subsubsection{Strong orthogonality}
\label{sssec:strong-orthogonality}
Finally, we introduce a notion of orthogonality of vectors that will be used in \Cref{ssec:zero-dim}, that is much stronger than the usual notion of orthogonality.

\begin{definition}
\label{def:strong-orthogonality}
Let $\Fn = \S_1 \oplus \dots \oplus \S_t$ be an orthogonal direct sum decomposition for $t$ orthogonal subspaces $\S_1, \dots, \S_t$. Let $\pi_i : \Fn \rightarrow \S_i$ denote the orthogonal projection map on $\S_i$, for all $1 \leq i \leq t$. Then two vectors $u, v \in \Fn$ are called \textit{strongly orthogonal} with respect to $\S_1, \dots, \S_t$ if and only if $\pi_i(u)$ is orthogonal to $\pi_i(v)$ for each $i$.
\end{definition}

It is important to note that if two vectors $u,v$ are strongly orthogonal with respect to $\S_1, \dots, \S_t$, then they are orthogonal (but the converse is not true). This is because the direct sum $\S_1 \oplus \dots \oplus \S_t = \Fn$, so we have $u = \sum_{i=1}^{t} \pi_i(u)$, and $v = \sum_{i=1}^{t} \pi_i(v)$, from which it follows that $u^\ast v = \sum_{i=1}^{t} (\pi_i(u))^\ast \pi_i(v)$, the other terms vanishing due to orthogonality of the subspaces, and finally by strong orthogonality we get $u^\ast v = 0$.

==> archive/scratch.tex <==
\section{Scratch}

%
%\title{A least squares objective function whose minimizers lie on low dimensional affine subspaces
%
%\title{A parameterized least squares problem whose minimizers lie on low dimensional affine subspaces

\begin{lemma} 
\begin{sloppypar}
Let $V \in \F^{n \times p}$ be semi-unitary and a basis for $\S$. Define $\MsymT(\S,\S') = \{A \in \Msym(\S,\S') \mid \rank{(V^\ast A V)} = p\}.$ Assume $n \geq 1$, $q \leq p$. Then
\end{sloppypar}
\begin{enumerate}[(i)]
    \item $\MsymT(\S,\S')$ is non-empty.
    % \item $\MsymT(\S,\S')$ is a smooth embedded submanifold of $\Sym{n}$ \green{LC: Sym(n) or Sym(n) s.t. T full rank ?} of dimension $\alpha\{n(n-1)/2-2p(n-p-q)\}+n.$
    \item $\MsymT(\S,\S')$ is a dense open subset of $\Msym(\S,\S').$
\end{enumerate}

\end{lemma}
\begin{proof}
\begin{enumerate}[(i)]
    \item Since $\Mpos(\S,\S') \subseteq \MsymT(\S,\S')$ and since $\Mpos(\S,\S')$ is non-empty from \Cref{lemma:existence}, $\MsymT(\S,\S')$ is non-empty.
    % \item This proof follows the proof of \Cref{lemma:embedding-Msym}, with $\alpha = 1$ if $\F = \R$ and $\alpha = 2$ for $\F = \C$. Define $\MsymT = \{A \in \Fnn \mid A \in \Sym(n), \rank{(A_{1:p,1:p})} = p, \rank{(A_{p+1:p+q,1:p})} = q, A_{p+q+1:n,1:p} = 0\}$.
    % The only difference lies in Step 1. We define $f(n,p,q) = \alpha \{ n(n-1)/2-2p(n-p-q) \} + n$. Let $\mathcal{U} \subseteq \R^{\alpha pq}$ be the set of $q\times p$ rank-$q$ matrices, and $\mathcal{V} \subseteq \R^{\alpha p^2}$ be the set of $p \times p$ rank-$p$ Hermitian matrices. Both sets are open. We then identify $\MsymT$ with $\mathcal{U} \times \mathcal{V} \times \R^{\alpha(n-p)(n-p-1)/2+(n-p)}$, an open subset of $\R^{f(n,p,q)}$. The rest of the proof is unchanged.
    %
    \item
    Let $\MsymT = \{A \in \Sym{n} \mid \rank{(A_{1:p,1:p})} = p,  \rank{(A_{p+1:p+q,1:p})} = q,  A_{p+q+1:n,1:p} = 0\}$.
    $\MsymT(\S,\S')$ is clearly open since the set of rank-$p$ matrices is open and so is $\Msym(\S,\S')$. \green{LC: probably missing a bit ?}
    To show density, consider any $A \in \Msym = \{A \in \Sym{n} \mid \rank{(A_{p+1:p+q,1:p})} = q, A_{p+q+1:n,1:p} = 0\}$. Let $T = A_{1:p,1:p}$. If $T \in \Gl{p}$, we are done. Assume $T \not\in \Gl{p}$. Since $\Gl{p}\cap\Sym{p}$ is dense within $\Sym{p}$, there exist $\{T_i\}_{i=1}^\infty$, $T_i \in \Sym{p}\cap\Gl{p}$ such that $T_i \to T$ as $i \to \infty$. Then define $A_i$ as $(A_i)_{kl} = (T_i)_{kl}$ if $1 \leq k,l \leq p$ and $(A_i)_{kl} = A_{kl}$ otherwise (i.e., $A_i$ is equal to $A$ except in the top-left $p \times p$ block where it equals $T_i$). Then $A_i \in \Sym{n}$, $\rank{((A_i)_{1:p,1:p})} = \rank{(T_i)} = p$ and $A_i \to A$ since $\|A_i - A\|_F^2 = \|T_i - T\|_F^2 \to 0$. So $\MsymT$ is dense within $\Msym$ and so $\MsymT(\S,\S')$ is dense within $\Msym(\S,\S')$.
\end{enumerate}
\end{proof}

This is analoguous to the usual tridiagonal decomposition build on the Lanczos process, i.e., \green{could be a bit superfluous}
\[ \begin{bmatrix} v_1^* \\ \vdots \\ v_k^* \\ v_{k+1}^* \\ \vdots \end{bmatrix} A \begin{bmatrix} v_1 & \dots & v_k & v_{k+1} & \dots \end{bmatrix} = \left[
    \begin{array}{ccc|c|c}
        \alpha_1 & \beta_2 &             &              &  \\
        \ddots   & \ddots  & \ddots      &              &  \\
                 & \beta_k & \alpha_k    & \beta_{k+1}  &  \\
        \hline
                 &         & \beta_{k+1} & \alpha_{k+1} &  \ddots \\
        \hline
                 &         &             & \ddots       &  \ddots \\
    \end{array}
    \right].
\]


First fix $u \in \Fp{q}$, and suppose there is a solution to \eqref{eq:sufficient-cond}. Combining the first two equations of \eqref{eq:sufficient-cond} gives $H (H^\ast H)^{-1} B^\ast u + \mu N t + \begin{bmatrix} 0 \\ z_{b,\omega,\mu}(t) \end{bmatrix} = G_\omega N t'$, from which it follows that $H^{\ast} G_\omega^{-1} \left ( H(H^\ast H)^{-1} B^\ast u + \mu Nt + \begin{bmatrix} 0 \\ z_{b,\omega,\mu}(t) \end{bmatrix} \right ) = 0$. By applying \Cref{lemma:HTSH} we immediately obtain that $d_{b,\omega,\mu} = (H^\ast H)^{-1} B^\ast u$. 

The argument for the converse already appears before. Assume now $d_{b,\omega,\mu} = (H^\ast H)^{-1} B^\ast u$ (such a $u$ exists by \Cref{thm:main_result}). Then by \Cref{lemma:HTSH} there exists $t$ satisfying \eqref{eq:equivalent-system-eqs}. Also, from the proof of \Cref{thm:main_result} there exists $t'$ such that $H d_{b,\omega,\mu} = N(\omega t' - \mu t) + \begin{bmatrix} 0 \\ z'_{b,\omega,\mu}(t,t')\end{bmatrix}$, which together with the second equation of \eqref{eq:equivalent-system-eqs} imply \eqref{eq:sufficient-cond}.

Let $V$, $V'$ be semi-orthogonal s.t. $\Img{V} = \S$ and $\Img{\begin{bmatrix} V & V' \end{bmatrix}} = \S'$. 
Also let $W = \begin{bmatrix} V & V' & V''\end{bmatrix}$ be orthogonal.
Then
\[ M(\S, \S') = \{ W A W^* \mid \rank{A_{21}} = q, A_{31} = 0 \}. \]

The choice of basis $W$ does not matter as $V$ and $V'$ can always be scaled on the right without changing $\rank{A_{21}}$ and keeping $A_{31} = 0$.

Clearly, $M(\S, \S')$ is an open set, since the set of rank-$q$ matrices is open. 
We can parametrize $M(\S, \S')$ by $A$. So we have
\[ M = W A W^* \]
We have $\vec{W A W^*} = (W \otimes W)\vec{A}$.
Restricting $A_{31} = 0$ means we have only $n^2-p(n-p-q)$ parameters.
Clearly the map as a $\F^{n^2-p(n-p-q)} \to \F^{n^2}$ is linear in the entries $\vec{A}$. 
Furthermore, $W \otimes W$ is full-rank since
$(W \otimes W)\vec{X} = 0$ if and only if $W X W^* = 0$ if and only if $X = 0$. So $W \otimes W$ is full-rank, and so is its restriction when $A_{31} = 0$ (this just excludes some columns from $W \otimes W$.
Since the map is full rank and linear, it's derivate is a constant full rank matrix.

When restricting ourselves to $\Gl{n}$, it doesn't really change anything: it's an open set intersecting another open set, so it's open. So nothing in the analysis before changes.

For Hermitian matrices,
\[ M(\S, \S') = \{ W A W^* \mid \rank{A_{21}} = q, A_{31} = 0, A = A^* \}. \]
Again, 
\[ \vec{WAW^*} = (W \otimes W) \vec{A} \]
with $W \otimes W$ full rank.
The condition $A_{31} = 0$ drops columns, so its still full-rank.
Since $A = A^*$, varying $a_{ij}$ needs to also vary $a_{ji}$. The contribution of $a_{ij}$ and $a_{ji} = a_{ij}^*$ in the output $(W \otimes W) \vec{A}$ is
\[ a_{ij} (W_{:i} \otimes W_{:j}) + a_{ij}^* (W_{:j} \otimes W_{:i}) = a_{ij} (v_i \otimes v_j) + a_{ij}^* (v_j \otimes v_i) \]
But we know $W \otimes W$ is orthogonal. Meaning for $(i,j) \neq (x,y)$, $(v_i \otimes v_j)^* (v_x \otimes v_y) = 0$. 
So in particular for $(i,j)$ (say $i \geq j$) and $(x,y)$ (say $x \geq y$) with $(i,j) \neq (x,y)$ (hence $(i,j) \neq (y,x)$), the columns associated with $a_{ij}$ ($(v_i \otimes v_j)$ and $(v_j \otimes v_i)$) and $a_{xy}$ ($(v_x \otimes v_y)$ and $(v_y \otimes v_x)$) are all pairwise orthogonal. 
Then writing $a_{ij} = a_{ij}^R + i a_{ij}^I$ we have
\[ a_{ij} (v_i \otimes v_j) + a_{ij}^* (v_j \otimes v_i) = (v_i \otimes v_j + v_j \otimes v_i) a_{ij}^R + i (v_i \otimes v_j - v_j \otimes v_i) a_{ij}^I \]
So we see that the image associated with $a_{ij}$ and with $a_{xy}$ are orthogonal.
